Render for CNN: Viewpoint Estimation in Images Using CNNs Trained with Rendered 3D Model Views

Object viewpoint estimation from 2D images is an essential task in computer vision. However, two issues hinder its progress: scarcity of training data with viewpoint annotations, and a lack of powerful features. Inspired by the growing availability of 3D models, we propose a framework to address both issues by combining render-based image synthesis and CNNs. We believe that 3D models have the potential in generating a large number of images of high variation, which can be well exploited by deep CNN with a high learning capacity. Towards this goal, we propose a scalable and overfit-resistant image synthesis pipeline, together with a novel CNN specifically tailored for the viewpoint estimation task. Experimentally, we show that the viewpoint estimation from our pipeline can significantly outperform state-of-the-art methods on PASCAL 3D+ benchmark.

==> tex/approach.tex <==
We first introduce our formulation of the 3D detection problem. Then, we introduce how we synthesize millions of highly diverse images from a large-scale 3D model set. Finally, we introduce how we use a training set containing real images and many more synthetic images to learn a deep CNN specifically tailored for 3D detection.
\subsection{Problem Formulation}
For an input RGB image, our goal is to estimate the azimuth of an object in a given bounding box. The bounding box can come from human annotation or any detection algorithm. 

% There are two standard formulations of this problem in literature: 1) the popular discrete viewpoint classification formulation, containing 8 to 24 discrete classes~\cite{Savarese_ICCV2007_Multiview,xiang2014beyond}, and 2) the recent continuous viewpoint regression formulation~\cite{massa2014convolutional}. Both formulations have their merits and drawbacks. The first one can output multiple viewpoint hypotheses and their confidences, which can be important for future processing, but the output is coarsely discretized. The second one outputs a finer-grained estimation, but it can only output a single viewpoint prediction with no confidence. 

We propose to formulate the problem as a \emph{fine-grained view} classification problem, by evenly discretizing the azimuth angles into 360 bins and elevation angles into 180 bins. Compared with traditional coarse-fined classification formulation, typically containing 8 to 24 discrete classes~\cite{Savarese_ICCV2007_Multiview,xiang2014beyond}, this formulation is more accurate; compared with regression-based formulations~\cite{xxx}, it also captures viewpoint ambiguities, possibly caused by symmetry or occlusion patterns, which are useful for future processing. For such a fine-grained formulation, the challenge is that more training samples are needed. This, however, is not a problem for us since we can render a large number of images.


\subsection{System Overview}

The pipeline of our system has two stages: the training data synthesis stage and the CNN learning stage. 

In the training data generation stage, we synthesize a large amount of images by rendering from 3D models and post-processing operations. % These synthetic data can be combined with real data to form a training set. 
The synthesis process is controlled by a set of parameters. The parameters are sampled from a coarsely defined distribution, in contrast to existing methods that use fixed pre-defined parameters~\cite{Aubry14} or seek ``optimal'' parameters with heavy computation~\cite{rozantsev2015rendering}. We use a simple, highly scalable strategy, thus enabling the synthesis of massive amounts of images with highly diverse appearances. Since all our models have been pre-aligned automatically, we automatically obtain a viewpoint annotation from the rendering parameters at no human cost.

In the CNN learning stage, we learn a 360-way viewpoint classifier by fine-tuning a pre-trained CNN model. We feed this deep neural network with the large amount of synthetic data generated in the previous stage.

% ---- ---- ---- ---- %
% ---- SYNTHESIS ---- %
% ---- ---- ---- ---- %
\subsection{Image Synthesis for Training}
\label{sec:synthesis}
Our synthesis process is fully automatic and thus highly scalable. 


Instead of optimizing rendering parameters locally, we add lots of perturbations to the synthesis process (e.g., random light positions, camera pose variations, cropping). 

The motivation for this is to prevent the deep neural network from picking up unreliable patterns and pushing it to learn more robust features for viewpoint estimation.

The synthesis involves four steps: model normalization, rendering, background synthesis, and cropping. We discuss them step by step in the following. For representative output images of the synthesis process see Figure~\ref{fig:synthetic_images}.

\paragraph{Model normalization} As Figure~\ref{fig:dataset} shows, our models are already aligned by orientation and placed on the ground plane. We normalize each 3D model to have unit (1) radius by isotropic scaling. Then, we move the model center to the origin of the world coordinate system.

\paragraph{Rendering} The parameters that affect the rendering include camera location, pose and lighting condition. To render each image, we sample a set of these parameters from a distribution as follows:

\begin{itemize}\denselist
\item {\bf Lighting condition}. We add 4 point lights. All lighting parameters are sampled i.i.d. The position $p_{light}$ is uniformly sampled on a sphere of radius $14.14$, between latitude $0\deg$ and $60\deg$; the energy $E \sim \mathcal{N}(4,3)$; the color is fixed to be white. 

\item {\bf Camera extrinsics.} We first describe the camera position parameters (i.e., translation parameters). In the polar coordinate system, let $\rho$ be the distance of the optical center to the origin, $\theta$ and $\phi$ be the longitude and latitude, respectively. $\rho$ is sampled from a truncated Gaussian $\mathcal{N}(7, 3)$ with a lower threshold $6$. $\phi$ is sampled from a truncated Gaussian $\mathcal{N}(15\deg, 15\deg)$, with an upper threshold $90\deg$ and lower threshold $-10\deg$. We propose two strategies to sample $\theta$: 1) uniformly sample from $[0\deg, 360\deg)$, and 2) sample from a distribution estimated from a training dataset. The two strategies are compared in the experiment section.

We then describe the camera pose parameters (i.e., rotation parameters). We randomly perturb the y-axis of the image plane pointing upward by an in-plane rotation, sampled from $\mathcal{N}(0, 5)$. Then we set the camera to look at the origin, the image plane perpendicular to the ray from the optical center to the origin. 

\item {\bf Camera intrinsics.} The focal length and aspect ratio are fixed to be $35$ and $1.0$, respectively.
\end{itemize}

We use Blender~\cite{blender}, an open-source 3D graphics and animation software, to efficiently render each 3D model. % We use the "Blender Render" engine in rasterization mode. %(ray-tracing disabled)

\paragraph{Background synthesis} Images rendered as above have a fully transparent background, and the object boundaries are very sharp. If we use such data for training, the learned classifier is likely to overfit to unrealistic boundary patterns. Therefore, we synthesize the background with a simple, scalable approach. For each rendered image, we randomly sample an image from SUN397, an existing scene database. We use alpha-composition to blend a rendered image as  foreground and a scene image as background. We randomly set the image center offset between the two images with a uniform distribution. 

\paragraph{Cropping} Since our goal is to estimate the viewpoint of an object in a bounding box, the last step of synthesis is to crop the image. We first compute a tight bounding box of the object through its mask, then we randomly stretch and shrink the box. For the general case, we adjust the left, right, top and bottom side of the box using the same set of parameters, by adding a normal random variable proportional to its width or height. For the specific case of chair viewpoint estimation, we also try to actively crop more bottom parts since chair legs and seats are often occluded. % Note that a more sophisticated way to determine crop parameters is to study the statistics of occlusion and truncation in the training set, which requires a segmentation mask and whole object area annotation (including occluded and truncated parts).



% In terms of machine time cost, rendering 128 images for each of the 6928 chair models ($6928 \times 128 = 886,784$ images in total) on one Intel Xeon 3.2GHz 24-core server in parallel takes around 6 hours. Synthesizing the backgrounds and cropping images take approximately another hour. Thus data generation for near 1 million rendered images takes around 7 hours in total.

\begin{figure}[t]
	\includegraphics[width=\linewidth]{./fig/rendering_examples.eps}
	\caption{Synthetic image examples}
	\label{fig:synthetic_images}
\end{figure}



\subsection{Network Learning}
\label{sec:network}
To effectively exploit this synthesized large-scale dataset, we need a model with sufficient learning capacity. CNNs are the natural choice for this challenge. We learn a fine-grained object viewpoint classifier using a CNN. We evenly discretize the azimuth angle to 360 classes and use a CNN to classify the viewpoint to one class.

We train a CNN using a fine-tune approach, similar to~\cite{girshick2014rich}. The pretrained model is from RCNN~\cite{girshick2014rich}, which has 5 convolutional layers and 3 fully connected layers, plus one softmax loss layer. The weights are trained from ImageNet. We fix the first few layers and fine tune upper layers with viewpoint labeled training images, which can be real images, synthetic images, or both. For each fine-tuned model, we search for hyperparameters that work well for the scale of the problem. We pick the model with highest validation accuracy for testing. It takes around 6 to 12 hours for our model to converge with Caffe~\cite{jia2014caffe} running on a Tesla C-series GPU.

% \paragraph{Remark} We choose RCNN for two reasons. Firstly, the focus of this work is to explore and analyze an 3D model image synthesis-based viewpoint estimation system, rather than network architecture tuning. In this sense, RCNN fits our demand due to its popularity and public availability, so that all our results can be easily produced, even though better architectures may lead to further performance improvement. Secondly, RCNN is effective for 2D detection; therefore, its convolutional layers can be shared across 2D detection and viewpoint estimation to achieve 3D detection.
 
% We also want to note the specialty of our problem in the context of transfer learning, if real images and rendered images are regarded as two domains. In classical transfer learning experiments of CNN features, features learned on task A is fine-tuned and used on task B. For example, features learned from ImageNet classification challenge can be transferred to PASCAL VOC detection challenge. , 


%\begin{figure*}[t]
%\begin{center}
%    \includegraphics[width=0.9\linewidth]{./fig/finetune}
%\end{center}
%   \caption{Fine tune RCNN trained from ImageNet data. Transfer knowledge learnt from rendered images to natural images.}
%\label{fig:finetune}
%\end{figure*}d

==> tex/dataset.tex <==
\label{sec:dataset}
\begin{figure}[t!]
\includegraphics[width=\linewidth]{./fig/aligned_chairs.eps}
\caption{Some example automatically aligned 3D chairs in our dataset}
\label{fig:dataset}
\end{figure}

The training data of our system is synthesized from a large 3D chair model dataset with orientation alignment. 

Our dataset contains 6,928 3D meshes of chair models. % should refer to shapenet synset after the TR is released
All our models are downloaded from the ``chair'' subtree of ShapeNet, which provides extensively annotated 3D models in a hierarchical categorization according to WordNet synsets, similar to ImageNet. We further manually cleaned these downloaded models, by removing those that contain more than a single chair instance. The final number of 6,928 3D meshes is obtained after this manual clean-up.

% second, what is orientation alignment, show examples in a figure, how it is done, what is the computation complexity.

We establish a consistent orientation among chair models, following the automated scheme proposed by~\cite{huang2013fine}. Examples of aligned chair models are shown in Figure~\ref{fig:dataset}. Our  manual inspection shows that the alignment is near-perfect, i.e., humans do not find misalignments of more than 10$^{\circ}$ between 1000 sampled pairs of models. % The automatic alignment program takes about half an hour to run.

Since these models have a consistent alignment, we obtain viewpoint annotations automatically at rendering. This is a big advantage over human annotation: it takes seconds for a person to label the viewpoint of an object coarsely, for example, up to 16 discrete bins. More accurate viewpoint annotation becomes very difficult for humans.

==> tex/futurework.tex <==

\begin{itemize}
\item with / without b.box detection (iccv)
\item render with / without occlusion (iccv)

\item chair only vs many categories (cvpr vs iccv)
\item 80K vs millions of renderings (cvpr)
\item texture / without texture (iccv)
\item with / without bounding blur, motion blur (iccv)
\item render only / render + real (cvpr+iccv)
\item generalizability (iccv)
\end{itemize}




==> tex/supp_requirement.tex <==


Authors may optionally upload supplementary material, which may not fit in the PDF size limit and may include:
videos to showcase results/demo of the proposed approach/system that were ready at the time of paper submission, but could not be included in the body of the paper due to reasons of format,
images, tables and other results that were ready at the time of paper submission, but could not be included in the body of the paper due to reasons of space,
anonymized related submissions to ICCV or other conferences and journals, and
appendices or technical reports containing extended proofs and mathematical derivations of results that are presented in the paper but could not be included due to reasons of space and are not essential to the understanding of the submitted paper.
ICCV encourages authors to submit videos using an MP4 codec such as DivX contained in an AVI. Also, please submit a README text file with each video specifying the exact codec used and a URL where the codec can be downloaded.

The authors should refer to the contents of the supplementary material appropriately in the paper. Note that reviewers will be encouraged to look at it, but are not obligated to do so. Please note that:

The paper for review (PDF only) must be submitted first before the supplementary material (PDF or ZIP only) can be submitted.
All supplementary material must be self-contained and zipped into a single file. The following formats are allowed: avi, doc, docx, mp4, pdf, wmv. CMT imposes a 100MB limit on the size of this file. Note that you can update the file by uploading a new one (the old one will be deleted and replaced).
Please make sure that the supplementary material directly supports the paper as submitted prior to the paper deadline. ONLY results generated by the algorithm/approach/system reported in the submitted version are allowed. Material based on improvements subsequent to the paper deadline is not allowed. In particular, new experiments on new datasets, new experiments on the same datasets obtained by using new parameters or by re-training the model are NOT allowed.
Do not submit a newer version of the paper as supplementary material. A newer version of the paper or portion thereof, with description of an improved algorithm/approach/system or even one spelling or typo correction, is not allowed.
